Effective Discovery of Meaningful Outlier Relationships

We propose PODS (Predictable Outliers in Data-trendS), a method that, given a collection of temporal data sets, derives data-driven explanations for outliers by identifying meaningful relationships between them. First, we formalize the notion of meaningfulness, which so far has been informally framed in terms of explainability. Next, since outliers are rare and it is difficult to determine whether their relationships are meaningful, we develop a new criterion that does so by checking if these relationships could have been predicted from non-outliers, i.e., if we could see the outlier relationships coming. Finally, searching for meaningful outlier relationships between every pair of data sets in a large data collection is computationally infeasible. To address that, we propose an indexing strategy that prunes irrelevant comparisons across data sets, making the approach scalable. We present the results of an experimental evaluation using real data sets and different baselines, which demonstrates the effectiveness, robustness, and scalability of our approach.

==> removed.tex <==
June 7

%As discussed in Section~\ref{sec:problem-definition}, 

The scatterplot in Figure~\ref{subfig:intro-scatterplot}, for example,
depicts all possible z-score alignments for temperature and heating
complaints. These alignments are then used to devise a linear \trend,
i.e., the solid line crossing the plotted points.
%
For simplicity, we refer to the general alignment of scores of two attributes as \textit{attribute alignment}.
%
\hide{Note, however, that if two attributes do not have a single pair of aligned outliers, \tipo trivially does not need to align their scores: there is no
outlier alignment to be explained. }


To avoid tackling alignments across ranges of timestamps, we propose a strategy to boost scores that were already computed whenever relevant cumulative 
effects are present.
%
In summary,
%
\jf{Do evaluate the effectiveness of this approach?} \ab{there are experiments comparing the initial scores and the dominant scores}
%
As illustrated in the rainfall example in
Section~\ref{sec:intro}, a regular value $x^i$ preceded by high values
(stormy days) should be assigned a proportionally  higher score $u^i$
to reflect the \textit{lingering, cumulative effects} of the outlier events
that occurred prior to it.


----------------------------------------------------------------------
The  investigation of
relationships between \textit{aligned outliers}, i.e., outliers that
either co-occur or occur close by in time, can also help users to more judiciously
clean data. 
%
Typically, outliers are removed or smoothed in order to become acceptable values~\cite{dasu2003}.
%
However, when outliers are not data errors and carry relevant semantic
information, it is important to keep them in the data to avoid
statistical distortions~\cite{dasu@kdd2014}.
%
\hide{\jf{Maybe we need a better way to describe 'unreliable'}}
%
Domain knowledge is required to determine whether outliers should be
cleaned. In practice, however, for large data or analyses that involve
multiple data sets whose quality may be undependable, this can be challenging.
%
In this context, the detection of relationships between outliers from
different data sets can provide useful information and a potential
explanation for the outlier, indicating that it may correspond to a
real event.
% be a useful tool to gather more information
%about the outliers themselves. This, in turn, can help users take
%decisions as to whether the outliers should be cleaned.


%
Consider the example in Figure~\ref{subfig:intro-raw}. A user could
smooth the first heating complaint peak in October (circled in black)
to make it more similar to previous values in the same month.
%, as it is so abruptly different. 
However, by contrasting this peak with the
aligned temperature in the bottom graph (circled in black), we notice
that the drop in temperature \textit{explains} the complaint peak,
increasing its probability of being a meaningful, real-world event
instead of a data error.
%
Note that outlier alignments \textit{should be
  statistically meaningful} in order to be useful as a data science
tool: if the alignments are merely coincidental, lacking statistical
robustness, they cannot be trusted as a means to better understand
outliers.
%

There are many challenges involved in
discovering meaningful outlier alignments. %
First, an event (reflected in data as an outlier) may influence (or be
influenced by) other events that occur within close-by time
intervals. For example, if it rains heavily for a few days, effects of
the abnormal rainfall can be felt even after it subsides. It is thus
important to take into account extreme values that may not be
perfectly aligned in time, otherwise relevant explanations may be
missed.
%
\hide{\jf{If the green lines connect different days, why are they vertical?
could this be represented differently? could we put the day number to
make it clearer?; and what do the lines in b) mean?} \ab{I added day numbers. It is the fastest solution for now}}
%
In Figure~\ref{subfig:intro-raw}, for example, blue solid lines
connect values from different data sets that occur on the same day, and the 
green dashed line connects values that occur on slightly different
days (December 13 and 14, circled in green).

\hide{\jf{What is the value for Pearson here?} \ab{if we add a number,
    it can be complicated to explain: when using points with small
    mean residuals, below 1 and above -1, which correspond to most
    days, the correlation is around -0.44 (not very strong, but not
    close to zero either). If you look at Figure 1a, there is
    correlation for most winter months.  So maybe what we should say
    here is that the warmer months conceal a relationship that is far
    stronger, involving aligned outliers in colder months. By the way,
    in the SIGMOD paper we dismissed Pearson with synthetic data.}}
%
%\todo{The 
%  normalized/standardized Pearson correlation coefficient is XXXX}.
%

%
\hide{\ab{Talking about Pearson here is not very relevant because it
    makes no sense to contrast Pearson over all points with Pearson
    over a very small sample. The point we are trying to make here is
    that a relationship over extreme alignments does not need to be
    the same that we observe when we take the data as a whole. Here,
    in the extremes there are peaks aligned with drops; on the whole
    data, there is a slice where the temperature keeps varying but the
    number of complaints stops dropping. If dismissing Pearson more
    emphatically is crucial, we can use the synthetic example we had
    in the SIGMOD paper.}}
%
\hide{\jf{should we refer to fig 1(b) which shows the correlation
    between the outliers?} \ab{I don't think so, because in Fig 1b
    there is a long trend encompassing things --- it's not only over
    the outliers. Again, I believe that it's best to say that the true
    relationship between outliers is very very strong and negative,
    and using the data as a whole conceals it because of warmer
    months. I'm not sure we need to present any actual numbers here.}}

%% However, if we take into account only the days with abnormally high
%% numbers of complaints, there is a clear relationship with aligned 
%% large drops in temperature.
%The blue lines, in particular, correspond to outliers co-occurring in the
%same days. %\ab{Challenge 1: is this clear relationship meaningful, though?}
%

\paragraph{Problem Statement.} 

\hide{\jf{need to improve the flow -- this sounds a bit repetitive}}

\textit{statistically meaningful relationships across their aligned 
  outliers}.  For simplicity, we refer to these relationships as 
\textit{meaningful outlier alignments}.

As previously stated, the relationship between unusual events that are temporally aligned
can serve as an explanation for the outliers, \textit{as long as these alignments are meaningful}. 
%
Such explanations, in turn, can help inform data-driven  decisions,
be it the design of policies and interventions or data cleaning. %% \ab{I think it's less repetitive now. In
%% the paragraph above, we just say that the relationships can work as explanations, but don't make the need
%% for stat. meaningfulness explicit.}

\hide{\ab{While previous approaches have been proposed to identify outlier relationships in
specific contexts~\cite{bailis2017macrobase,chirigati@sigmod2016,roy@vldb2015,wu2013scorpion,zhang@edbt2017},
our focus on whether these relationships are \textit{statistically
 meaningful} is, to the best of our knowledge, novel. \ab{they have, but not over incredibly small samples of outliers.}}}

\hide{
\jf{Are the items below providing too much detail? Should we instead
  provide a higher-leverl overview here? Also, we have 3 challenges
  but 4 bullets, and then, in Section 3, we have 3 subsections. Could
  we align these? Maybe, we should have the description in regular
  text instead of itemized bullets} \ab{I don't think we are giving too much detail, but enough to understand the
  method and the connection with the images. In the past, I believe we had agreed on using bullets because some reviewers doubted that we had
  enough contributions, and this makes it clearer. Also, not all contributions necessarily match one challenge: the weighting scheme helps with many
  things, from statistical significance to guaranteeing that the behavior assigned to aligned outliers does not have to agree with the overall behavior.
   I'd leave it as-is.}}

----------------------------------------------------------------------


\hide{However, urban data sets are published in portals which
provide limited search capabilities -- often keyword-based interfaces
over their contents and metadata. While these queries are
effective for unstructured data, there are new opportunities and
challenges involved in searching for relevant structured data.}
% JF: not sure we want to talk about bring data together from 
% multiple portals since we are not really emphasizing scalability
% In addition, data are spread over a large number of sites....
% but we can argue that even in NYC, data sets are spread --
% NYCOPendata, MTA, are all in different places
%
\hide{We envision a new generation of search engines that allow users to
issue a rich set of complex queries over large collections of
structured data sets and that take advantage of the structure
inherent in the data.
}

\hide{ JF: this should appear later to improve the flow
In particular, these decisions may be based on
extreme data values that %, which potentially
indicate anomalous real events. %that should be addressed.
%be indicators of real, abnormal events.
}
%
%In th paper, we  focus on decisions that are informed by extreme data values, which can 
%be indicators of real, abnormal events. %behaviors. 
%represented by outliers in data sets. 
%Extreme values and outliers  are indicators of unusual behavior.
%

%
%
%In this paper, we focus on the problem of discovering relationships
%among a large number of data sets that materialize under extreme
%conditions.
%
%Extreme values and outliers  are indicators of unusual behavior.
%

\hide{". . there seems something else in life besides time, something
  which may conveniently be called “value," something which is
  measured not by minutes or hours but by intensity, so that when we
  look at our past it does not stretch back evenly but piles up into a
  few notable pinnacles, and when we look at the future it seems
  sometimes a wall, sometimes a cloud, sometimes a sun, but never a
  chronological chart – E.M. Foster"}

\hide{
In statistical analysis, methods are often applied to reduce the
influence of outliers~\cite{encyc-stat-2005}. 
%% Consider, for example,
%% Winsorization~\cite{encyc-stat-2005}, which makes the mean
%% of a given sample more robust by replacing the $k$ smallest
%% and largest values with values in between, i.e., given a sequence with
%% $n$ items, the values in the interval $[0,k-1]$ are replaced with
%% values in $[k,2k-1]$, and values in the interval $[n-k,n]$ are
%% replaced with $[n-2k,n-k]$.
%
However, as Tukey pointed out~\cite{tukey-1960}, treating outliers as
\emph{strays} 
%or \emph{wild shots} 
leads to a critical pitfall: one ends up working with ideal values
\emph{``which ought to have been provided''}, instead of considering the values actually provided.
%
When we encounter an outlier during data analysis, we must discern whether the value 
reflects a real event or a data quality issue. If we determine that the outlier is indeed a data
quality issue, the outlier can be removed or properly repaired. 
%But if the outlier
%is a correct value,
Otherwise, removing it or attenuating its contribution will
fundamentally alter the data and subsequent analysis results.
%
Therefore, it is critical to distinguish strays from proper 
values~\cite{freire@deb2016}.
}

% Later
\hide{
Recently, techniques have been proposed to both detect and
explain outliers. 
%
Since manually inspecting large data sets (or large data collections) is time
consuming, a number of approaches have been proposed to automatically
sift through data, filter, aggregate, and highlight
outliers and potentially interesting
features~\cite{chandola2009anomaly, vartak2014seedb, doraiswamy@tvcg2014}.
%
Others have focused on the problem of identifying causes and deriving
explanations for outliers~\cite{chirigati@sigmod2016,bailis2017macrobase,zhang@edbt2017,wu2013scorpion,roy@vldb2015}.
%
These have either considered explanations that include categorical
attributes or that

When one encounters outliers in a data set (or query result)
 $O_A$ in a data set $A$, if
another data set $B$ is identified whose outliers co-occur with $O_A$,
$O_B$ can serve as an explanation for $O_A$ 
}


%
\hide{ % JF moved up
We frame our problem %% of determining whether an outlier reflects a real
%% event
as the detection of \textit{meaningful} co-occurrences between
\textit{outliers} in different data sets, in which case the
outliers are said to be explained.
}
%

\hide{Essentially, an outlier from \todo{data set} $A$ co-occurs with  one from \todo{data set} $B$ if they share the same temporal 
reference -- i.e., they occurred in the same hour, day, etc. Furthermore, \todo{co-occurrences between outliers are 
 meaningful if they are predictable, correlated, and not coincidental}. A formal definition of the problem is provided in Section~\ref{preliminary-approach-overview}. 
 \ab{Change data sets $A$ and $B$ to attributes}
}




\hide{
\jf{We need to get the speed data and the number of fatalities: https://visionzeronetwork.org/resources/speed-fatality-map}

\jf{use heating complaints and point to nytimes article on people living in projects without proper heating -- create more food, more space}

\jf{ask aline for 311 heat complaints and temperature --
create Jupyter notebook:
plot 1:
the actual data values (number of complaints and temperature);
plot 2:  mean residuals for complaints and temperatures; x axis should
show month or seasons}
}

\hide{ 
- C3  Data come in different units. It is hard to relate the absolute number of complaints and temperature values

- C1 Since, by definition, there are relatively few outliers, one important
challenge is how to obtain confidence in outlier-based relationships,
and how to help an expert discern whether a relationship makes sense
or if it is coincidental. ; if we  increase the number of points and using all data, correlation may disappear

- C2 Need to examine multiple granularities to cover a comprehensive set
  of outliers. For example, when  there is an abrupt increase in the number of
  heating complaints, if this number is not high globally, it is not
  considered an outlier.  Different time windows capture different trends/events. For
  example, in the middle of the winter, a temperature drop  from
  30 to 20F often does not lead to
  problems;
  but a similar drop during the fall, when heating units are not yet
  operational does (can we see this in the data?)

}

\hide{
\ab{Don't know if this is one of the challenges... We don't focus much on scalability} Given the growing number of data sets that 
are available and the fact
that relationships materialize under many different conditions, even
if we address the aforementioned challenges, 
discovery through manual inspection clearly does not scale. \ab{Also: Given the growing number of data sets that are available and the fact
that relationships materialize under many different conditions, even
if we address the aforementioned challenges, 
discovery through manual inspection clearly does not scale.}
}

\hide{
 It \emph{normalizes} attribute values so that co-occurring
  outliers can be properly detected and compared. Attributes are
  normalized using a variation of \textit{mean residual normalization}
  (standardization of variables) \cite{CRR73}: each point is
  standardized with respect to preceding time windows of different
  sizes. This has important benefits. First, the technique is
  data-driven and does not require \textit{per attribute} numerical
  thresholds to determine which values are outliers. Therefore, it can
  be applied, automatically, to a large number of data sets.
%
%% In addition, when dealing with
%% time-varying data, it is important to capture outliers that
%% represent local and global events.
  In addition, the use of windows of varying size makes the approach
  flexible and able to capture outliers that represent both local and global events.
%%% changing as per Parni's suggestion
%% detect a variety of outliers, and consequently,
%%   capture relationships that represent both seasonal and global
%%   patterns. 
  For example, contrast
  Figures~\ref{subfig:intro-raw-scatter} and
  \ref{subfig:intro-norm-scatter}: in \ref{subfig:intro-raw-scatter},
  which shows the co-occurring raw values, no clear trend can be
  observed, while in~\ref{subfig:intro-norm-scatter}, which uses
  window sizes of 30 days to normalize both temperature and heating
  complaints, we can see the outliers (red triangles) coming. Also
  note that while the value for day D2 appears as an inlier
  in~\ref{subfig:intro-raw-scatter}, it is an outlier in
  \ref{subfig:intro-norm-scatter} for both
  axes. %, i.e., it represents a co-occurring outliers for temperature and heating complaints.
%
As we discuss in Section~\ref{general-components}, we search for
relationships using a range of time window sizes.
\hide{by varying the
    time-widow size, it is possible to capture shorter and longer-term
    outliers, and consequently, discover a range of relationships.}
}
%
 %Moreover, the technique enables
  %the detection of a comprehensive set of outliers that capture both
  %seasonal context and global behaviors. 

%\jf{articulate that this normalization takes into account different
%  time windows -- making the approach flexible and able to capture
%  different patterns}

%\itemspace 


%% The intuition is that meaningful co-occurrences
%% between outliers start taking shape across values that
%% lie close to them, and thus, these values should be
%% given a higher weight in the regression models.

%% \jf{Need to re-state what the problem is -- intuition must come before
%%   describing the approach-- just adding points may
%%   lead to detect correlation that does not explain the outliers. To
%%   identify relevant points that explain the outliers,  we....}
%% %
%% To accomplish this, we
%%   \emph{propose a new strategy based on weighted linear regression
%%     models}~\cite{CRR73} that ensures a better fit for co-occurring
%%   values that are either outliers or are close to outliers. 

%% \ab{I think we have to deeply convince readers that this
%%     intuition is useful and hard to question... We mention it a lot on
%%     the paper, but it never feels super ``final''} \jf{don't we have a
%%     figure that illustrates this?} \ab{we do, but I don't know if examples are the most adequate tool to convince here. Maybe a logical argument?}
% This can be said in section 3 -- should be more concise here
%, which is 
% equivalent to performing a join operation using the timestamps as  key. Pairs with no 
% co-occurring outliers are pruned away; otherwise, 
    
%

%% The
%%   intuition is that meaningful co-occurrences between outliers start
%%   taking shape across values that lie close to them, and thus, these
%%   values should be given a higher weight in the regression
%%   models. \ab{I think we have to deeply convince readers that this
%%     intuition is useful and hard to question... We mention it a lot on
%%     the paper, but it never feels super ``final''} \jf{don't we have a
%%     figure that illustrates this?} \ab{we do, but I don't know if examples are the most adequate tool to convince here. Maybe a logical argument?}

% \itemspace 

\hide{
\item Once co-occurrences are detected, it performs a statistical test
  to prune the ones that are coincidental. The remaining
  co-occurrences are further examined to assess whether they represent
  a correlation between attributes. To accomplish this, we
  \emph{propose a new strategy based on weighted linear regression
    models}~\cite{CRR73} that ensures a better fit for co-occurring
  values that are either outliers or are close to outliers. The
  intuition is that meaningful co-occurrences between outliers start
  taking shape across points that lie close to them, and thus, these
  points should be given a higher weight in the regression models.
% \todo{The quality of the regression models dictates whether or not correlations can be detected.}


  \item If the regression models detect correlations, to \emph{assess
      the meaningfulness of the correlations}, the framework verifies
    whether the correlations serve as evidence for the outlier
    co-occurrences, i.e., if the correlations can be used to predict
    the outliers.  Intuitively, \tipo verifies if the models can see
    co-occurrences between outliers coming.

}

%Consider, for example, urban data. 
%
Increasingly, cities around the world are collecting data that capture
information about the different components of urban
environments~\cite{barbosa@bigdata2014,opendata@book2013,chicagoopendata,nycopendata,sfoopendata,parisopendata,rioopendata}. By
exploring this data exhaust and discovering relationships between
indicators coming from distinct datasets, we can obtain insights that
inform policies, make cities more efficient, and improve their
residents’ lives.
%

%
Often, as these examples illustrate, actions are taken

As cities around the world are increasing capturing data that capture
different aspects of urban
environments
%


